Interactive configurator with FO(.) and IDP-Z3

Industry abounds with interactive configuration problems, i.e., constraint solving problems interactively solved by persons with the assistance of a computer. The computer program, called a configurator, needs to perform a variety of reasoning tasks with the (often incomplete) information that the user provides. Imperative programming approaches make such systems difficult to implement and maintain. Knowledge-based configurators have been proposed to help engineers solve such problems, but many challenges remain. We present IDP-Z3, a new reasoning engine for the FO(.) KR language, and we report on its use for building configurators automatically from a knowledge base.

==> kr.tex <==

\section{Introduction (start of template)}

The \textit{KR2022 Proceedings} will be printed from electronic
manuscripts submitted by the authors. These must be PDF (\emph{Portable
Document Format}) files formatted for US letter paper (8-1/2$''$ $\times$ 11$''$).

\subsection{Length of Papers}

For the main conference track and additional tracks/sessions, except for the
\emph{Recent Published Research Track}, we invite two types of paper
\emph{submissions}:
\begin{itemize}
\item Full papers of up to 9 pages, including abstract, figures, and appendices
  (if any), but excluding references and acknowledgements.
\item Short papers of up to 4 pages, including abstract and figures, but excluding
 references and acknowledgements.
\end{itemize}

For the \emph{Recently Published Research Track} we invite submissions consisting
of:
\begin{itemize}
\item a cover page (single page) listing the title, the authors, a complete
  reference to the original paper, and a public or privately accessible url
  from which the paper can be downloaded, and
\item an extended abstract of the paper of either one page (preferred) or two
  pages, following the format for regular KR2022 paper submissions.
  % The abstract should present the main contributions of the paper, discuss
  % the relevance of the paper to KR, and explain the significance of the
  % results.
\end{itemize}

If your paper is accepted, please carefully read the notifications you receive,
and check the proceedings submission information
website\footnote{\url{https://kr.proceedings.confdna.com/info}} for up-to-date
information. That website holds the most updated information regarding the
Camera Ready Version.

\subsection{Word Processing Software}

As detailed below, KR has prepared and made available a set of
\LaTeX{} macros and a Microsoft Word template for use in formatting
your paper. If you are using some other word processing software, please follow the format instructions given below and ensure that your final paper looks as much like this sample as possible.

\section{Style and Format}

\LaTeX{} and Word style files that implement these instructions
can be retrieved electronically.

\subsection{Layout}

Print manuscripts two columns to a page, in the manner in which these
instructions are printed. The exact dimensions for pages are:
\begin{itemize}
\item left and right margins: .75$''$
\item column width: 3.375$''$
\item gap between columns: .25$''$
\item top margin---first page: 1.375$''$
\item top margin---other pages: .75$''$
\item bottom margin: 1.25$''$
\item column height---first page: 6.625$''$
\item column height---other pages: 9$''$
\end{itemize}


\subsection{Format of Electronic Manuscript}

For the production of the electronic manuscript, you must use Adobe's
\emph{Portable Document Format} (PDF). A PDF file can be generated, for
instance, on Unix systems using \texttt{ps2pdf} or on Windows systems
using Adobe's Distiller. There is also a website with free software
and conversion services: \url{http://www.ps2pdf.com}. For reasons of
uniformity, use of Adobe's \emph{Times Roman} font is strongly suggested.
In \LaTeX2e{} this is accomplished by writing
\begin{quote}
  \texttt{\textbackslash{}usepackage\{times\}}
\end{quote}
in the preamble.\footnote{You may want also to use the package
 \texttt{latexsym}, which defines all symbols known from the old \LaTeX{}
 version.}

Additionally, it is of utmost importance to specify the \texttt{letter} format
(corresponding to 8-1/2$''$ $\times$ 11$''$) when formatting the paper. When
working with \texttt{dvips}, for instance, one should specify \texttt{-t
 letter}.

\subsection{Title and Author Information}

Center the title on the entire width of the page in a 14-point bold font. The
title must be capitalized using Title Case. Below it, center author name(s) in
12-point bold font. On the following line(s) place the affiliations, each
affiliation on its own line using 12-point regular font. Matching between
authors and affiliations can be done using numeric superindices. Optionally, a
comma-separated list of email addresses follows the affiliation(s) line(s),
using 12-point regular font.

% \subsubsection{Blind Review}

% In order to make blind reviewing possible, authors must omit their names and
% affiliations when submitting the paper for review. In place of names and
% affiliations, provide a list of content areas. When referring to one's own
% work, use the third person rather than the first person. For example, say,
% ``Previously, Gottlob~\shortcite{gottlob:nonmon} has shown that\ldots'',
% rather than, ``In our previous work~cite{gottlob:nonmon}, we have shown
% that\ldots'' Try to avoid including any information in the body of the paper
% or references that would identify the authors or their institutions. Such
% information can be added to the final camera-ready version for publication.
% You cannot include author names in your submitted PDF metadata. Any paper
% breaking this rule may be desk rejected without review.

\subsection{Abstract}

Place the abstract at the beginning of the first column 3$''$ from the
top of the page, unless that does not leave enough room for the title
and author information. Use a slightly smaller width than in the body
of the paper. Head the abstract with ``Abstract'' centered above the
body of the abstract in a 10-point bold font. The body of the abstract
should be in typeset in a 9-point font.

The abstract should be a concise, one-paragraph summary describing the
general thesis and conclusion of your paper. A reader should be able
to learn the purpose of the paper and the reason for its importance
from the abstract. The abstract should be no more than 200 words long.

\subsection{Text}
 
The main body of the text immediately follows the abstract. Use 10-point type
in a clear, readable font with 1-point leading (10 on 11).

Indent when starting a new paragraph, except after headings.

\subsection{Headings and Sections}

When necessary, headings should be used to separate major sections of your
paper. (These instructions use many headings to demonstrate their appearance;
your paper should have fewer headings.). All headings should be capitalized
using Title Case.

\subsubsection{Section Headings}

Print section headings in 12-point bold type in the style shown in these
instructions. Leave a blank space of approximately 10 points above and 4 points
below section headings. Number sections with arabic numerals.

\subsubsection{Subsection Headings}

Print subsection headings in 11-point bold type. Leave a blank space of
approximately 8 points above and 3 points below subsection headings. Number
subsections with the sec- tion number and the subsection number (in arabic
numerals) separated by a period.

\subsubsection{Subsubsection Headings}

Print subsubsection headings in 10-point bold type. Leave a blank space of
approximately 6 points above subsubsection headings. Text follows the
subsubsection in the same line after a double space, like in this paragraph
itself. Do not number subsubsections.

\subsubsection{Acknowledgements}

You may include an unnumbered acknowledgments section, including
acknowledgments of help from colleagues, financial support, and permission to
publish. If present, acknowledgements must be in a dedicated, unnumbered
section appearing after all regular sections but before any appendices or
references.

Use
\begin{quote}
  \texttt{\textbackslash{}section*\{Acknowledgements\}})
\end{quote}
to typeset the acknowledgements section in \LaTeX{}.

\subsubsection{Appendices}
Any appendices directly follow the  main text and look like sections, exceptthat they are numbered with capital letters in-
stead of arabic numerals. See this document for an example.

\subsubsection{Supplementary Material}
Authors may optionally provide supplementary material (e.g. proof details, additional experimental results)
as a separate file. Such material will be consulted at the discretion of reviewers and will not be published.
Please refer to the conference website for further information.

\subsubsection{References}

The references section is headed ``References'', printed in the same
style as a section heading but without numeration. A sample list of
references is given at the end of these instructions. Use a consistent
format for references. The reference list should not include unpublished
work.

\subsection{Citations}


Citations within the text should include the author's last name and
the year of publication, for example~cite{gottlob:nonmon}.  Append
lowercase letters to the year in cases of ambiguity.  Treat multiple
authors as in the following examples:~cite{abelson-et-al:scheme}
or~cite{bgf:Lixto} (for more than two authors) and
cite{brachman-schmolze:kl-one} (for two authors).  If the author
portion of a citation is obvious, omit it, e.g.,
Nebel.  Collapse multiple citations as
follows:~cite{gls:hypertrees,levesque:functional-foundations}.
nocite{abelson-et-al:scheme}
nocite{bgf:Lixto}
nocite{brachman-schmolze:kl-one}
nocite{gottlob:nonmon}
nocite{gls:hypertrees}
nocite{levesque:functional-foundations}
nocite{levesque:belief}
nocite{nebel:jair-2000}

\subsection{Footnotes}

Place footnotes at the bottom of the page in a 9-point font.  Refer to
them with superscript numbers.\footnote{This is how your footnotes
should appear.} Separate them from the text by a short
line.\footnote{Note the line separating these footnotes from the
text.} Avoid footnotes as much as possible; they interrupt the flow of
the text.

\section{Illustrations}

Place all illustrations (figures, drawings, tables, and photographs) throughout
the paper at the places where they are first discussed, rather than at the end
of the paper.

They should be floated to the top (preferred) or bottom of the page, unless
they are an integral part of your narrative flow. When placed at the bottom or
top of a page, illustrations may run across both columns, but not when they
appear inline.

Illustrations must be rendered electronically or scanned and placed directly in
your document. They should be cropped outside \LaTeX{}, otherwise portions of the
image could reappear during the post-processing of your paper. All
illustrations should be understandable when printed in black and white, albeit
you can use colors to enhance them. Line weights should be 1/2-point or
thicker. Avoid screens and superimposing type on patterns, as these effects may
not reproduce well.

Number illustrations sequentially. Use references of the following
form: Figure~1, Table~2, etc. Place illustration numbers and captions
under illustrations. Leave a margin of 1/4-inch around the area
covered by the illustration and caption.  Use 9-point type for
captions, labels, and other text in illustrations. Captions should always appear below the illustration.

\section{Tables}

Tables are considered illustrations containing data. Therefore, they should also appear floated to the top (preferably) or bottom of the page, and with the captions below them.

\begin{table}
\centering
\begin{tabular}{lll}
\hline
Scenario  & $\delta$ & Runtime \\
\hline
Paris       & 0.1s  & 13.65ms     \\
Paris       & 0.2s  & 0.01ms      \\
New York    & 0.1s  & 92.50ms     \\
Singapore   & 0.1s  & 33.33ms     \\
Singapore   & 0.2s  & 23.01ms     \\
\hline
\end{tabular}
\caption{Latex default table}
\label{tab:plain}
\end{table}

\begin{table}
\centering
\begin{tabular}{lrr}
\toprule
Scenario  & $\delta$ (s) & Runtime (ms) \\
\midrule
Paris       & 0.1  & 13.65      \\
            & 0.2  & 0.01       \\
New York    & 0.1  & 92.50      \\
Singapore   & 0.1  & 33.33      \\
            & 0.2  & 23.01      \\
\bottomrule
\end{tabular}
\caption{Booktabs table}
\label{tab:booktabs}
\end{table}

If you are using \LaTeX, you should use the \texttt{booktabs} package, because
it produces better tables than the standard ones. Compare Tables
\ref{tab:plain} and~\ref{tab:booktabs}. The latter is clearly more readable for
three reasons:

\begin{enumerate}
\item The styling is better thanks to using the \texttt{booktabs} rulers
  instead of the default ones.
\item Numeric columns are right-aligned, making it easier to compare the
  numbers. Make sure to also right-align the corresponding headers, and to use
  the same precision for all numbers.
\item We avoid unnecessary repetition, both between lines (no need to repeat
  the scenario name in this case) as well as in the content (units can be shown
  in the column header).
\end{enumerate}

\section{Formulas}

KR's two-column format makes it difficult to typeset long formulas. A usual
temptation is to reduce the size of the formula by using the \texttt{small} or
\texttt{tiny} sizes. This doesn't work correctly with the current \LaTeX{}
versions, breaking the line spacing of the preceding paragraphs and title, as
well as the equation number sizes. The following equation demonstrates the
effects (notice that this entire paragraph looks badly formatted):
%
\begin{tiny}
\begin{equation}
    x = \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i
\end{equation}
\end{tiny}%

Reducing formula sizes this way is strictly forbidden. We \textbf{strongly}
recommend authors to split formulas in multiple lines when they don't fit in a
single line. This is the easiest approach to typeset those formulas and
provides the most readable output%
%
\begin{align}
    x =& \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \nonumber\\
    + & \prod_{i=1}^n \sum_{j=1}^n j_i
\end{align}%

If a line is just slightly longer than the column width, you may use the
\texttt{resizebox} environment on that equation. The result looks better and
doesn't interfere with the paragraph's line spacing: %
\begin{equation}
\resizebox{.91\linewidth}{!}{$
    \displaystyle
    x = \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i
$}
\end{equation}%

This last solution may have to be adapted if you use different equation environments, but it can generally be made to work. Please notice that in any case:

\begin{itemize}
\item Equation numbers must be in the same font and size than the main text
  (10pt).
\item Your formula's main symbols should not be smaller than {\small small}
  text (9pt).
\end{itemize}

For instance, the formula
%
\begin{equation}
    \resizebox{.91\linewidth}{!}{$
    \displaystyle
    x = \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j
$}
\end{equation}
%
would not be acceptable because the text is too small.

\section{Examples, Definitions, Theorems and Similar}

Examples, definitions, theorems, corollaries and similar must be written in
their own paragraph. The paragraph must be separated by at least 2pt and no
more than 5pt from the preceding and succeeding paragraphs. They must begin
with the kind of item written in 10pt bold font followed by their number (e.g.:
Theorem 1), optionally followed by a title/summary between parentheses in
non-bold font and ended with a period. After that the main body of the item
follows, written in 10 pt italics font (see below for examples).

In \LaTeX{} we strongly recommend you to define environments for your examples,
definitions, propositions, lemmas, corollaries and similar. This can be done in
your \LaTeX{} preamble using \texttt{\textbackslash{}newtheorem} -- see the
source of this document for examples. Numbering for these items must be global,
not per-section (e.g.: Theorem 1 instead of Theorem 6.1).

\begin{example}[How to write an example]
Examples should be written using the example environment defined in this template.
\end{example}

\begin{theorem}
This is an example of an untitled theorem.
\end{theorem}

You may also include a title or description using these environments as shown in the following theorem.

\begin{theorem}[A titled theorem]
This is an example of a titled theorem.
\end{theorem}

\section{Proofs}

Proofs must be written in their own paragraph separated by at least 2pt and no
more than 5pt from the preceding and succeeding paragraphs. Proof paragraphs
should start with the keyword ``Proof." in 10pt italics font. After that the
proof follows in regular 10pt font. At the end of the proof, an unfilled square
symbol (qed) marks the end of the proof.

In \LaTeX{} proofs should be typeset using the \texttt{\textbackslash{}proof}
environment.

\begin{proof}
This paragraph is an example of how a proof looks like using the
\texttt{\textbackslash{}proof} environment.
\end{proof}


\section{Algorithms and Listings}

Algorithms and listings are a special kind of figures. Like all illustrations,
they should appear floated to the top (preferably) or bottom of the
page. However, their caption should appear in the header, left-justified and
enclosed between horizontal lines, as shown in
Algorithm~\ref{alg:algorithm}. The algorithm body should be terminated with
another horizontal line. It is up to the authors to decide whether to show line
numbers or not, how to format comments, etc.

In \LaTeX{} algorithms may be typeset using the \texttt{algorithm} and
\texttt{algorithmic} packages, but you can also use one of the many other
packages for the task.

\begin{algorithm}[tb]
\caption{Example algorithm}
\label{alg:algorithm}
\textbf{Input}: Your algorithm's input\\
\textbf{Parameter}: Optional list of parameters\\
\textbf{Output}: Your algorithm's output
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $t=0$.
\WHILE{condition}
\STATE Do some action.
\IF {conditional}
\STATE Perform task A.
\ELSE
\STATE Perform task B.
\ENDIF
\ENDWHILE
\STATE \textbf{return} solution
\end{algorithmic}
\end{algorithm}

\section*{Acknowledgments}

The preparation of these instructions and the \LaTeX{} and Bib\TeX{}
files that implement them was supported by Schlumberger Palo Alto
Research, AT\&T Bell Laboratories, and Morgan Kaufmann Publishers.
Preparation of the Microsoft Word file was supported by IJCAI.  An
early version of this document was created by Shirley Jowell and Peter
F. Patel-Schneider.  It was subsequently modified by Jennifer
Ballentine and Thomas Dean, Bernhard Nebel, Daniel Pagenstecher,
Kurt Steinkraus, Toby Walsh, and Carles Sierra. The current version
has been prepared by Marc Pujol-Gonzalez, Francisco Cruz-Mencia, and Diego
Calvanese.

\appendix

\section{\LaTeX{} and Word Style Files}
\label{stylefiles}

% The \LaTeX{} and Word style files are available at
% \begin{center}
%   \url{https://kr2021.kbsg.rwth-aachen.de/downloads/KR22_authors_kit.zip}.
% \end{center}
% These style files implement the formatting instructions in this document.

The \LaTeX{} style file is \texttt{kr.sty} and the Bib\TeX{} style file to use
is \texttt{kr.bst}.  The \LaTeX{} file \texttt{kr-instructions.tex}, containing
the source of the present document, and the Bib\TeX{} file
\texttt{kr-sample.bib}, containing some example Bib\TeX{} entries, may serve as
a formatting sample (these two files are not needed for typesetting your
paper).  The \LaTeX{} style file is for version 2e of \LaTeX{}, oand the
Bib\TeX{} style file is for version~0.99c (\emph{not} version~0.98i) of
Bib\TeX{}.  Note that the \texttt{kr.sty} style file differs from the
\texttt{kr.sty} file used for KR2020 but remains unchanged since then.

The Microsoft Word style file consists of a single file, \texttt{kr21.docx},
which may serve as a formatting sample for Microsoft Word users.  Please make
use of the ad-hoc styles that have been defined for the different parts of the
document, and that are listed in the Styles Pane.  Note that this template
differs from the one used for KR2020, but remains essentially unchanged since then.

Further information on using these styles for the preparation of papers for
KR2022 can be obtained by contacting
\href{mailto:kr.proceedings@confdna.com}{kr.proceedings@confdna.com}.


==> sections/_old_CaseStudies.tex <==
% No separate section on case studies is needed. Info on SG & FM is moved to evaluation instead.
% DO NOT DELETE!
\section{Case studies}
\label{sec:cases}

In this subsection, we summarise four previously published case studies that use IDP-Z3 as a reasoning engine.

\subsection{Machine Component Designer}

\citeauthor{Aerts2022} (\citeyear{Aerts2022}) describe the creation of an IDP-based knowledge base system for the design of machine components, implemented in collaboration with a multinational company.
This company employs engineers worldwide to conceive ``design-to-order'' components.
Before the collaboration, each engineer followed their own \textit{ad hoc} design process, mostly based on their own experience and preferences.
This approach has multiple downsides: (a) designing a component consumes a large amount of time, (b) engineers may choose sub-optimal designs, and (c) if a senior engineer leaves, a great deal of knowledge is lost by the company.

To overcome these issues, the design knowledge was formalized through a series of knowledge extraction workshops.
In such a workshop, both knowledge engineers and domain experts are involved in modeling the knowledge used when designing machine components.
Each workshop spanned a few days, and was performed in geologically different branches of the company, to ensure diversity in the knowledge.

Initially, the DMN standard was used to create a model of the experts' knowledge.
While DMN was found to be intuitive, it was unable to represent all knowledge in a straightforward manner.
Indeed, DMN is well suited for rule-based, hierarchical decision procedures with one unique output, but it is not suitable for reasoning when several choices are possible.
For example, to find the optimal design of the component, the user had to make tentative design choices, determine the resulting cost, backtrack, and subsequently consider alternative designs.

In \fodot parlance, we would say that DMN can represent definitions, but not axioms.
Axioms are used to exclude designs that are not feasible.
To allow the addition of axioms on top of the rule-based logic, the DMN model was converted into an \fodot KB.
%Here, further knowledge workshops were held to flesh out these constraints.
Additionally, some \textit{preferences} were added: e.g., ``always use the cheapest material possible.''
Using a weighted sum, these preferences can then be used to automatically determine the optimal design for any given circumstances.

In total, the KB contains 10 parameters describing 60 different materials (such as a maximum temperature of steel) and 27 parameters for 31 components (such as torque and maximum pressure).

The Interactive Consultant (described in the previous section) is used to allow interaction with the KB.
It is configured for this application by simply changing the \fodot KB.
Besides the standard interactions, the interface was further extended to fit the company's specific needs.
Examples of such extensions are a functionality to compare two designs, an extended version of explanations in which not only the set of choices are shown but also the underlying constraints (which has since been added to the IC), a way to deactivate and reactivate certain axioms, and an integration with a Machine Learning algorithm that suggests designs based on historic data.

Overall, the company and its engineers are very positive about the tool.
Besides a reported daily time-save of up to 30 minutes for each engineer, they report other benefits to its usage.
First and foremost, it leads to more ``first-time right'' designs, which lowers production time and cost.
Secondly, for new engineers the tool serves as an excellent learning tool, allowing them to indirectly learn from the knowledge of the more experienced engineers.
For more experienced engineers on the other hand, the tool is used to challenge their assumptions: when in doubt, they can swiftly verify if their initial ideas are correct.
Lastly, with their knowledge captured in a KB, engineers leaving will not result in loss of knowledge for the company.

The functionality of the original IDP3-based tool was somewhat limited because IDP3 is not able to perform floating point calculations.
To overcome this, it has recently been ported over into IDP-Z3, to benefit from its support of arithmetic.


%\textbf{Interesting aspects:}
%\begin{itemize}
%    \item Created two tools: one DMN based, one IDP (later cDMN) based
%    \item Interactive Consultant to interact with knowledge
%    \item Uses multiple existing inference tasks:
%    \begin{itemize}
%        \item Propagation, relevance, explanation, model expansion, optimization, relevance
%    \end{itemize}
%    \item Also added custom inference tasks:
%    \begin{itemize}
%        \item Comparison, Extended Explanation (which is now ``normal'' explanation)
%        \item[$\rightarrow$] latter might be nice example of how feedback from use cases is incorporated to general system?
%    \end{itemize}
%    \item Tool was also extended with Machine Learning for historic designs
%    \item ``Finally, the IDP-system is not able to perform floating point calculations.'' $\rightarrow$ This has been solved using IDP-Z3
%    \item Also propose cDMN
%\end{itemize}
%
%\textbf{Advantages of the tool:}
%\begin{itemize}
%    \item Tool can be used to challenge assumptions
%    \item Improved consistency and accuracy in designs
%    \item More ``first time right'' designs, leading to lower production time and cost
%    \item Daily time-save of up to 30 minutes
%    \item Useful for both new and experienced engineers
%\end{itemize}

\subsection{Adhesive Selection Tool}

%\textit{Work submitted, acceptance notification 15th of Jan.}
Together with the Flanders Make Joining \& Materials Lab we have been working on a case study concerning adhesive selection \cite{Jordens2021}.

In industry, the usage of glues is rising in popularity due to their favorable characteristics.
However, besides some superficial, vendor-locked websites, there is no tooling available to support selecting the right adhesive for the right use case.
Adhesives come in a wide range of options, categorised into 18 different adhesive families, with none suitable for all applications.
The selection of an adhesive is based on which substrates are used (e.g., steel, wood, plastics, $\ldots$) and on bond requirements such as minimum strength, maximum elongation, operating temperature range and more.

To begin, we held multiple knowledge workshops in order to create a KB.
Instead of using DMN to create the initial model, as in the previous case, we used cDMN due to the constraint-heavy nature of the problem domain.
In total, we identified and formalised 21 adhesive parameters (such as bond strength, adhesion and temperature range) and 11 substrate parameters (such as solvent resistance, maximum temperature and magnetic type).
The current version of the KB contains 55 individual adhesives, and 31 substrates.

An interesting aspect of this case is how missing data is handled: if a parameter value is not known (because it was, e.g., not listed in the adhesive's data sheet), the tool assumes the value of the adhesive's family.
In this way, the tool uses a reasonable estimate of the real value, similar to what the experts do.
However, if the family's value is also unknown, the tool warns the user that the value is unknown and it does not apply any constraints to that parameter, instead asking the expert to verify it manually.

The adhesive experts interact with the KB through the Interactive Consultant, allowing them to benefit from all of its features.
In particular, it allows reasoning in any direction.
While generally, the goal is to select an adhesive, in other cases, the adhesive is known, as well as one of the substrates, and the goal is to find a suitable second substrate.
%It is worth noting that the knowledge can not only used for the selection of an (optimal) adhesive.
%Indeed, though rare, there are cases in which the adhesive is already known (e.g., left over from a previous gluing task) and one substrate is already predefined, in which the goal is to find a second suitable substrate.
This ``substrate selection'' task is performed without modifying the KB in any way.

%\textit{(We are also planning on adding intensional reasoning here, but this was not described in the submitted work)}

Overall, the first impressions by the experts are positive.
In an initial test, the tool has reduced the selection process from 3 hours to 5 minutes for one especially difficult case.
While it seemed that the tool would be most useful for newer members of the J\&ML lab, the most experienced member has indicated that they can also benefit from it.
Indeed, this member typically chooses from a (limited) set of adhesives of which they know most properties by heart.
Using the tool, they can find out if there are any other adhesives which might be better suited for a job.


\subsection{Intelli-Select}
\label{sec:intelli-select}

\citeauthor{Deryck2021} (\citeyear{Deryck2021}) present their work on Intelli-Select\footnote{\url{https://www.intelli-select.com/}}, a tool created for international financial institutions to support investment management.
This tool combines Constrained Natural Language (CNL) and the IDP-Z3 system, to offer a user-friendly way for a customer to define his \textit{investment profile}.  
An investment profile is a set of rules that specify the financial assets that they consider eligible for investment.
This investment profile is created in CNL, and later converted to \fodot for processing.

For example, a user can construct the CNL sentence ``Equities issued in Germany are eligible'' to allow all German equities.
Additionally, a free-form Natural Language (NL) interface is also available, which suggests CNL equivalents.
Here, an NL sentence such as ``I would like to invest in German equities'' would be translated into the CNL statement shown earlier.

To create the KB, the CNL statements are represented in \fodot in the form of two definitions: one for eligibility, and one for ineligibility.
In the application, the IDP-Z3 system is then used to perform several reasoning tasks.
Firstly, each time a user adds new (in)eligibility rules, the system performs \textbf{propagation} to show the effect of the new rules.
If a rule's effect is unexpected, or the user is unsure why it happened, they can invoke the \textbf{explanation} inference. 
When a profile is considered finished, \textbf{model expansion} can be performed to identify the eligible assets, i.e., those that satisfy the \textit{eligible} definition.
Moreover, using \textbf{optimization}, it is possible to calculate minimal cost combinations of these eligible assets.
% Finally, the \textbf{abstract model generation} inference serves as a way to compare two different financial profiles, and find concrete differences.

%\begin{itemize}
%    \item Model expansion, to decide on the eligibility of assets
%    \item Optimization, to find minimal cost combinations of assets
%    \item Propagation, to show the effect of a new rule
%    \item Explanation, to explain an (in)eligibility
%    \item Abstract model generation, to compare two profiles
%\end{itemize}

Besides these standard reasoning tasks, the collaborating company requested a way to automatically convert the financial profile into a long and complex document with a specific format.
This document, called \textit{Appendix A}, is used both as an appendix to the contract with the client, and as the formal input to one of the systems in place at the company.
Previously, the company created such document manually, a process which typically took a few months to complete.
However, because the required knowledge of a financial profile is already present in the KB, we were able to add a specific method to automatically generate these documents in a few seconds, as described by \citeauthor{DeryckThesis} (\citeyear{DeryckThesis}).


As lessons learned, the authors outline two things.
Firstly, they mention that compared to standard applications in the field of financial technology, their tool is low in maintenance due to the separation between domain knowledge and reasoning tasks.
Secondly, while the creation of a KB is typically a challenging task, the use of CNL is a good way of lowering the effort.


%\stodo{rephrase their lessons learned}

\subsection{Notary / Legislation}

%\begin{itemize}
%    \item Building the KB for the first time took 10 days
%    \item Amending it took 0.5 days
%    \item 9 out of 20 rules did not need to be changed, showing the modularity of KBP
%    \item Refined explanation and relevance, based on request of notary
%\end{itemize}

The fourth case study deals with registration duties on property purchases in Belgium.
It was originally presented by \citeauthor{Deryck2018} (\citeyear{Deryck2018}) and later extended by \citeauthor{Deryck2019} (\citeyear{Deryck2019}).
In Belgium, registration duties depend on many parameters, such as the location, the type of property, the characteristics of the buyer and the seller, and more.
At the time of the first publication, these duties were determined by 11 articles of law.
For this case, a collaboration with a notary was set up to ensure the correctness of the knowledge.

Initially, the knowledge engineer and domain expert worked together to create a DMN model of the legislation.
Here, the user-friendliness of DMN meant that it could be used as a ``common language'' between the two, leading to less formalization errors.
This is an important point, as the law field contains a great deal of complex jargon.
After the DMN model was finished, the knowledge engineer converted the tables into \fodot, ready to be used by the IDP system.
Together with the Interactive Consultant, this formed an easy-to-use application.
Note that standard DMN tools would not have been sufficient, as the notary required a tool that could reason with partial information and could optimise the cost of the duties.
In total, the formalization process took 10 person-days.

Later in 2018, the relevant law was simplified by the Belgian government.
In \cite{Deryck2019}, the KB is updated to reflect these changes, together with improvements to the Interactive Consultant as requested by the notary office.
While the change was the most significant change to the real estate sales law to have ever happened, updating the KB required only 0.5 person-days, due to the KB's modular nature.

This application has been ported to IDP-Z3, and is available online\footnote{\url{https://interactive-consultant.idp-z3.be/?file=registratie.idp}}.  
It takes advantage of the arithmetic capabilities of IDP-Z3 to calculate the tax amount due.

% Propagation
% Relevance
% Explanation

